Run-time Parameter Sensitivity Analysis Optimizations

Efficient execution of parameter sensitivity analysis (SA) is critical to allow for its routinely use. The pathology image processing application investigated in this work processes high-resolution whole-slide cancer tissue images from large datasets to characterize and classify the disease. However, the application is parameterized and changes in parameter values may significantly affect its results. Thus, understanding the impact of parameters to the output using SA is important to draw reliable scientific conclusions. The execution of the application is rather compute intensive, and a SA requires it to process the input data multiple times as parameter values are systematically varied. Optimizing this process is then important to allow for SA to be executed with large datasets. In this work, we employ a distributed computing system with novel computation reuse optimizations to accelerate SA. The new computation reuse strategy can maximize reuse even with limited memory availability where previous approaches would not be able to fully take advantage of reuse. The proposed solution was evaluated on an environment with 256 nodes (7168 CPU-cores) attaining a parallel efficiency of over 92%, and improving the previous reuse strategies in up to 2.8x.

==> motivating.tex <==
\textedit{

\section{Background}

This section describes the motivating application and the Region Template
(RT) framework used to deploy the application workflow for execution on
distributed systems.

\subsection{Motivating Application} \label{sec:app}

High-resolution microscopy imaging enables the study of disease at the cellular
and sub-cellular levels. Investigating the changes in morphology of structures
at this level using whole slide tissue specimens can lead to a better
understanding of disease mechanisms and a better assessment of response to
treatment. 

A contemporary digital microscopy scanner can capture from a tissue specimen a
whole slide image containing 20 billion pixels (using 40X objective
magnification) in a few minutes. An 8-bit color uncompressed representation of
this image is over 50GB in size. A scanner with a slide loader can generate
hundreds of images in one or two days. Advanced tissue scanning devices
are becoming more widely available at low price points for use in research and
health care settings. We expect that in the near future research projects will
be able to collect tens of thousands of images per study. 

\begin{table}[htb!]
\begin{center}
\vspace*{-2ex}
\caption{Definition of parameters and range values: parameter space contains about 21 trillion points. }
%\vspace*{-2ex}
\begin{scriptsize}
\begin{tabular}{l l l l }
\hline
Parameter		& Description   					& Range Values			\\ \hline
%Target Image 		& Normalization target image 				& $[Img1,...,Img4]$ 		\\ \hline
B/G/R  			& Background detection thresholds 			&  $[210,220,...,240]$ 	\\ \hline
T1/T2			& Red blood cell thresholds				& $[2.5,3.0,...,7.5]$		\\ \hline
\multirow{2}{*}{G1/G2}	& Thresholds to identify 				& $[5,10,...,80]$		\\ 
			& candidate nuclei					& $[2,4,...,40]$		\\ \hline
MinSize(minS)		& Candidate nuclei area threshold   			& $[2,4,...,40]$ 		\\ \hline
MaxSize(maxS)		& Candidate nuclei area threshold 			& $[900,..,1500]$		\\ \hline 
MinSizePl \\ (minSPL)	& Area threshold before watershed  			& $[5,10,...,80]$		\\ \hline
MinSizeSeg \\ (maxSS)	& Area threshold in final output			& $[2,4,...,40]$ 		\\ \hline 
MaxSizeSeg \\ (minSS)	& Area threshold in final output  			& $[900,..,1500]$		\\ \hline 
FillHoles(FH) 		& propagation neighborhood				& $[4$-conn$,8$-conn$]$		\\ \hline
MorphRecon(RC)		& propagation neighborhood				& $[4$-conn$,8$-conn$]$		\\ \hline
Watershed(WConn)	& propagation neighborhood				& $[4$-conn$,8$-conn$]$		\\ \hline
\end{tabular}
\end{scriptsize}
\label{tab:parameters}
\vspace*{-4ex}
\end{center}
\end{table}


%
%\begin{figure*}[htb!]
%\begin{center}
%\includegraphics[width=0.98\textwidth]{images/nucleiPipelineCur}
%\vspace*{-3ex}
%\caption{An example analysis pipeline: normalization, segmentation and feature computation stages are presented along with their cascade of internal operations.}
%\vspace*{-3ex}
%\label{fig:example-app}
%\end{center}
%\end{figure*}
 
A typical analysis workflow consists of normalization, segmentation, feature
computation, and final classification operations.  The three
first analysis stages (Figure~\ref{fig:example-app}) are typically the most
costly phases of an analysis. The segmentation step, for instance, has to
process billions of pixels in a high resolution image and can identify hundreds
of thousands of cells. The feature computation step computes 20-50 shape and
texture features for each segmented object. All operations on our three most
compute intensive stages have been implemented for CPU and Intel Phi. More
details on the internal operations of each application stage may be found in
our previous work~\cite{Teodoro:2014:CPA:2650283.2650645,kurc2015scalable}. 

The final classification phase is less compute expensive and will typically
involve the use of data mining algorithms on aggregated information. Some of
the targets in this phase include not only classifying tissue images according
to progression, but also to gain insights of the underlying biological
mechanisms that distinguish between disease subtypes.  The effectiveness of an
analysis workflow is often sensitive to input data and input parameters. This
can lead to concerns about the validity and robustness of extracted or
discovered morphological properties. The parameters of the segmentation stage
for the motivating workflow along with their description and range values
(selected by an application expert) are presented in
Table~\ref{tab:parameters}. The large number of parameters and associated
parameters space (21~trillion parameter sets) makes it evident that it would be
very hard for one to manually evaluate its sensitivity. This creates a demand for systematic
and automated approaches to quantify the impact of the parameters to the output
as is provided by SA studies. Since the segmentation is a critical step in the information
extraction, we focus our efforts on the evaluation of this stage of the SA.


}

